Finite amplitude wave propagation through bubbly fluids

The existence of only a few bubbles could drastically reduce the acoustic wave speed in a liquid. Wood's equation models the linear sound speed, while the speed of an ideal shock waves is derived as a function of the pressure ratio across the shock. The common finite amplitude waves lie, however, in between these limits. We show that in a bubbly medium, the high frequency components of finite amplitude waves are attenuated and dissipate quickly, but a low frequency part remains. This wave is then transmitted by the collapse of the bubbles and its speed decreases with increasing void fraction. We demonstrate that the linear and the shock wave regimes can be smoothly connected through a Mach number based on the collapse velocity of the bubbles.

==> Note.tex <==
Fig. 1 : Put (c) and (d) below (b)
Fig. 3(a) and (b) should be below Fig 2
Fig. 3(c) as Fig. 4

Focus on the fact that we have studied the transmission of shock wave through bubbly gelatin. Significant slow down of shock speed is seen in experiment and explained by simulation
